Sampling in Constrained Domains with Orthogonal-Space Variational Gradient Descent

Sampling methods, as important inference and learning techniques, are typically designed for unconstrained domains. However, constraints are ubiquitous in machine learning problems, such as those on safety, fairness, robustness, and many other properties that must be satisfied to apply sampling results in real-life applications. Enforcing these constraints often leads to implicitly-defined manifolds, making efficient sampling with constraints very challenging. In this paper, we propose a new variational framework with a designed orthogonal-space gradient flow (O-Gradient) for sampling on a manifold $\mathcal{G}_0$ defined by general equality constraints. O-Gradient decomposes the gradient into two parts: one decreases the distance to $\mathcal{G}_0$ and the other decreases the KL divergence in the orthogonal space. While most existing manifold sampling methods require initialization on $\mathcal{G}_0$, O-Gradient does not require such prior knowledge. We prove that O-Gradient converges to the target constrained distribution with rate $\widetilde{O}(1/\text{the number of iterations})$ under mild conditions. Our proof relies on a new Stein characterization of conditional measure which could be of independent interest. We implement O-Gradient through both Langevin dynamics and Stein variational gradient descent and demonstrate its effectiveness in various experiments, including Bayesian deep neural networks.

==> ICML22_orthogonal_SVGD (clean)/maintheory.tex <==


\section{Theoretical Analysis}\label{sec:theory}


We theoretically justify the convergence of O-Gradient in this section. To do so, we first describe the target measure as a conditioned measure $\Pi_0$, then derive its associated orthogonal-space Fisher divergence, and finally prove that O-Gradient converges to $\Pi_0$. 
\subsection{Conditioned measure and its Stein characterization}
First of all, conditioning on a zero-measure set is a challenging concept.
Assume we have a distribution $\Pi$ with density $\pi$. Let $A$ be a set with $\Pi(A)\neq 0$, then $\Pi(B|A) = \frac{\Pi(B\cap A)}{\Pi(A)}.$ However, if $\Pi(A) = 0$, this definition is ill-posed. 
Instead, a standard way to define a conditioned measure on a zero measure set is using disintegration theorem \citep{chang1997conditioning}. 
Let $\Pi_z(\,\cdot\,) = \Pi(\,\cdot\,| g(x) = z)$ be the measure such that 
\bbb
\label{eq:condmeas}
\E_\Pi[ f(x)] = 
\E_{z \sim \Pi^g} \E_{x\sim \Pi_z} [f(x)],~~\forall f,
\eee
where $\Pi^g$ is the pushforward measure of $\Pi$ under $g$. 
It is worth noting that $\Pi_0$ \emph{is not} the measure with Hausdorff density $\pi$ on $\calG_0$. Instead, under regularity conditions, $\Pi_0$ can also be defined through Hausdorff density $\pi(x)/|\nabla g(x)|$ on $\calG_0$, see Lemma 6.4.1 of \cite{simon2014introduction}.


One can also avoid this rather abstract definition, and consider 
an alternative definition which is more intuitive and Bayesian.  
Suppose we observe $z = g(x) + \sigma\xi$,  where $\xi\sim \normal(0,1)$. Under prior $x\sim\pi$, the posterior $\pi_{\sigma^2,z}(x) \propto \pi(x) \exp(-|z -g(x)|^2/2\sigma^2)$.   
Then we can show that $\Pi_z$ is the (weak) limit of $\pi_{\sigma^2,z}$ as $\sigma \to 0$, moreover, it satisfies  a \emph{Stein characterization of conditional measure}. We need  some regularity assumptions to state our results. 
   
\begin{mydef}\label{def:greg}
A density $q$ is $g$-regular if there is a constant $L$ such that for small enough $\eta>0$, 
\begin{equation}
\label{eq:greg}
|\E_{\xi\sim \mathcal{N}(0,1)}[q^g(z+\eta\xi)/q^g(z)]-1|\leq L\eta,\quad \forall z.
\end{equation}
\end{mydef}
Note that Eq.~$\eqref{eq:greg}$ holds if $q^g$ is a Lipschitz function. Moreover, while Definition~\ref{def:greg} requires Eq.~\eqref{eq:greg} to hold for all $z$, in practice we only concern $\Pi_0$, thus only need the equation to hold for $z$ near $0$. 

\begin{pro}
\label{pro:disint}
Suppose $\pi$ is $g$-regular. Then the weak   limit of $\pi_{\eta,z}(x)\propto \pi(x)\exp(-\frac1{2\eta} (g(x)-z)^2)$ 
as $\eta\to 0$ concentrates on $\calG_z$ and satisfies Eq.~\eqref{eq:condmeas}. Moreover, for each $z$,  
\bbb
\label{eq:projstein}
\E_{\Pi_z} \left [\stein_\pi \phi \right] =0,\quad \forall \phi\bot \nabla g. 
\eee
\end{pro}
The first part of Proposition \ref{pro:disint} also provides us with a way to sample $\Pi_z$, as we can sample a sequence of distribution $\pi_{\eta_k,z}$ with $\eta_k\to 0$. However, this method involves double loops and is usually much more expensive than single-loop algorithms.  

The second part of Proposition \ref{pro:disint} can be used to formulate an orthogonal-space Stein equation. Specifically, given a $q$ concentrated on $\calG_z$, we consider checking whether $\E_q [\stein_\pi \phi]$ is zero for $\phi\in \calH_\bot=\{\phi: \phi\bot \nabla g\}$, which is a necessary condition for $q=\Pi_z$. 
Notably, this equation is well defined in $\RR^d$ without using any parameterization of $\calG_z$. 



Compared with the standard Stein equation,  we add an additional restriction that  $\phi\in\calH_\bot$.
We argue such restriction is actually very natural. To see that, we note $\Pi_z$ is concentrated on $\calG_z$, so we should check  the Stein equation with vector field that ``live'' only on $\calG_z$, namely the tangent bundle $\mathcal{T} \calG_z$. Notably, if $\phi(x)\in \mathcal{T} \calG_z$, then $\phi(x)\bot \dd g(x)$, therefore it is natural to consider $\calH_\bot$. 


\subsection{Orthogonal-Space Fisher divergence}


Next we consider how to generalize Fisher divergence for constrained sampling. Since the orthogonal-space Stein equation can only discern discrepancy in $\calH_\bot$, it is natural to consider an orthogonal-space Fisher divergence 
\begin{equation}
\label{eq:projfisher}
F_{\bot}(q,\pi):=\|D(s_q-s_\pi)\|^2_{\calH},     
\end{equation}
where $D$ is the $\calH_\bot$-projection operator defined pointwisely using Eq.~\eqref{eq:projD}. Its easy to see $F_\bot$ is well defined for a density $q$ on $\RR^d$. But it remains unclear whether it can be used to measure the distance between $q$ and $\Pi_z$. 

To answer this question, we need some form of strong convexity conditions.
Recall that in the unconstrained case,  such conditions can be characterized by Poincar\'{e} inequalities (PI) when $\H$ is $L^2_q$, so we will focus on this setting. 
PI counterparts of SVGD remain an open question \cite{gorham2017measuring,duncan2019geometry}, 
which we hope to be addressed by future works.
 When constrained on $\calG_z$, PI's formulation involves gradients so it depends on the Riemannian metric used in  $\calG_z$. One natural choice of Riemannian metric is the metric inherited from $\RR^d$ which equals $\|D(x)\nabla f(x)\|$, since $D(x)$ is also the projection onto the tangent bundle of $\calG_z$. This leads to the following definition.

\begin{mydef}
$\Pi_z$ follows a $\kappa$-PI, if for any smooth $f$ on $\RR^d$, $\var_{\Pi_z} [f]\leq \kappa \E_{\Pi_z}[\|D\nabla f\|^2]$.
\end{mydef}
PI on Riemannian manifold has been studied in previous work~\citep{hebey2000nonlinear,li2006weighted}. In particular, Theorem 2.10 of \cite{hebey2000nonlinear} shows that PI holds for the Riemannian measure if the manifold $\calG_z$ is compact, and hence it also holds for any equivalent distributions.
But it is often hard to find the exact PI constant $\kappa$ for $\Pi_z$, especially if we are interested in a family of $\Pi_z$ with possibly discontinuous dependence on $z$.


\begin{pro}
\label{pro:meandiff}
Suppose that $\Pi_z$ satisfies $\kappa$-PI for $|z|\leq \delta$, and $q$ is supported on $\{x: |g(x)|\leq \delta\}$. Suppose also that $\Pi_z, q^g, \pi^g$ admit $C^1$ density functions.
Then for any function $f$ such that $|f|\leq 1$, the following holds
\begin{align*}
|\E_{q} [f]-\E_{\Pi_0} [f]|\leq &\sqrt{8\kappa\E_q [\|D(s_q-s_\pi)\|^2]} 
~+~ \max_{|z|\leq \delta} |\E_{\Pi_z} [f]-\E_{ \Pi_0} [f]|. 
\end{align*}
\end{pro}
In particular, Proposition \ref{pro:meandiff} shows that if we have a  $q$ such that it is 1) supported close to $\calG_0$ and 2) $F_\bot (q,\pi)$ is small, then $q$ is close to $\Pi_0$ in total variation. We can also interpret the bound alternatively as a decomposition of the difference between $q$ and $\Pi_0$: the first part measures the difference along $\calH_\bot$ directions and it is controlled by $F_\bot$; the second part measures the difference along $\nabla g$ direction, and it is controlled by the distance between $q$'s support  to $\calG_0$.

As a final remark, the orthogonal-space Stein equation \eqref{eq:projstein} and orthogonal-space Fisher divergence \eqref{eq:projfisher} can be applied to densities supported on $\RR^d$, and their formulations do not require information of $\calG_0$ such as parameterization and geodesic. Therefore, they can be used as very computationally friendly statistical divergence in practice. 



\begin{pro}
\label{pro:flow}
Suppose we apply $v_t=v_\sharp+Du$ with \eqref{eq:vsharp} and \eqref{eq:proju} to the density field $q_t$.
\begin{enumerate}
    \item Let $M_t=\max\{|g(x)|,x\in \text{supp}(q_t)\} $. Let $S_t$ be the solution of an ordinary differential equation $\dot{S}_t=-\psi(S_t).$ Suppose $S_0=M_0<\infty$, then $M_t<S_t$ a.s..
    \item Assume $\psi$ is differentiable  with derivative  $\dot \psi$.  Suppose $g$ is also smooth enough so that
    \begin{equation}
        \label{eq:regular}
        \left|\nabla g^T s_\pi+\Delta g-\frac{2\nabla g^T \nabla^2 g \nabla g}{ \|\nabla g\|^2}\right|\leq C_0\|\nabla g\|^2.
    \end{equation}
\end{enumerate}
Then the KL-divergence follows $\frac{d}{dt}\KL(q_t\|\pi)\leq -F_\bot(q_t,\pi)+\E_{q_t} [|\dot{\psi}(g)|]+C_0\E_{q_t} [|\psi(g)|\|\nabla g\|^2].$
\end{pro}
The first result shows that the support of $q_t$ will shrink towards $\calG_0$. But in order to avoid possible stagnation case, e.g. $\|g\|$ is too small, it is necessary to impose \eqref{eq:regular}. 
The second result provides us some hint on the choice of $\psi$. Note that under $q_t$ for large enough $t$, $g(x)$ will take values close to $0$, so we need $\psi(0)=\dot{\psi}(0)=0$. Since $\psi(x)$ should have the same sign with $x$,  one natural choice would be $\psi(y)=\alpha\text{sign}(y)|y|^{1+\beta}$.
\begin{thm}
\label{thm:grad}
Suppose we choose $\psi(y)=\alpha\text{sign}(y)|y|^{1+\beta}$ for an $\alpha>0,\beta\in (0,1]$ and the conditions of Proposition \ref{pro:flow} hold. Suppose also that $\KL(q_0,\pi)<\infty$ and $\|\nabla g(x)\|\leq D_0$ if $|\psi(x)|<M_0$,  then 
$M_T=O(T^{-\frac1\beta}),$
$\min_{t\leq T} F_\bot(q_t,\pi)=O(\log T/T)$.
The orthogonal-space Stein equality holds approximately, in the sense that for any $\phi(x)\bot \nabla g(x)$ and $\|\phi\|_{\H}=1$, 
$\min_{t\leq T}|\E_{q_t} \stein_{\pi} \phi|\leq \sqrt{F_\bot(q_t,\pi)}=O(\sqrt{\log T/T}).$
\end{thm}
Theorem \ref{thm:grad} shows that we can obtain a $q_t$ that is supported on $\calG_{[-\delta,\delta]}=\{x:|g(x)|\leq \delta\}$, while it has close to zero orthogonal-space Fisher divergence and the  Stein identity holds approximately on $\calH_\bot$. Combining it with Proposition \ref{pro:meandiff}, we have 
\begin{cor}
Under the conditions of Theorem \ref{thm:grad}, for a bounded $f$ with $\calH=L^2_q$, suppose
 $h_f(z)=\E_\pi [f|g(X)=z]=\E_{\Pi_z} [f]$ is Lipschitz with near $z=0$, then 
$\min_{t\leq T}|\E_{q_t} [f]-\E_{\Pi_0} [f]|\leq O(\sqrt{\log T/T}).$
\end{cor}




